Achieving Conversational Goals with Unsupervised Post-hoc Knowledge Injection

A limitation of current neural dialog models is that they tend to suffer from a lack of specificity and informativeness in generated responses, primarily due to dependence on training data that covers a limited variety of scenarios and conveys limited knowledge. One way to alleviate this issue is to extract relevant knowledge from external sources at decoding time and incorporate it into the dialog response. In this paper, we propose a post-hoc knowledge-injection technique where we first retrieve a diverse set of relevant knowledge snippets conditioned on both the dialog history and an initial response from an existing dialog model. We construct multiple candidate responses, individually injecting each retrieved snippet into the initial response using a gradient-based decoding method, and then select the final response with an unsupervised ranking step. Our experiments in goal-oriented and knowledge-grounded dialog settings demonstrate that human annotators judge the outputs from the proposed method to be more engaging and informative compared to responses from prior dialog systems. We further show that knowledge-augmentation promotes success in achieving conversational goals in both experimental settings.

==> camera-ready-todo.tex <==
TODOS
- 

==> files/reviews.tex <==
Title: Post-hoc Knowledge Injection in Generated Dialog using Gradient-based Inference
Authors: Bodhisattwa Prasad Majumder, Harsh Jhamtani, Taylor Berg-Kirkpatrick and Julian McAuley


============================================================================
                            REVIEWER #1
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
The paper applies the plug-and-play language model (PPLM) to knowledge-based dialog response generation tasks (i.e. goal-oriented dialogs and knowledge-grounded dialogs). By substituting the attribute model in the original PPLM with 1) a self-consistency classifier and 2) a bag-of-word knowledge adherence predictor, the new attribute model can provide gradients that make responses conform to 1) context and 2) knowledge, respectively. 

Automated evaluation for diversity and human evaluation for quality have been carried out on the MultiWOZ and the WoW corpora. The proposed method has significantly outperformed baseline models on both evaluations and both corpora, which suggests that the proposal is highly effective.

STRENGTHS:

* A simple, intuitive, and effective formulation of the new attribute model that makes generated responses conform to both context and knowledge (by combining a context-response consistency classifier and the BoW likelihood of knowledge snippet tokens).

* Extremely good results from automated and human evaluations.

WEAKNESSES:

* Automated evaluation for quality is completely missing. While automated evaluation is not reliable in open-domain dialog response generation, it is still very important in goal-oriented dialogs and knowledge-grounded dialogs since a proper response should largely reflect the correct knowledge. Automated metrics (e.g. inform/success/BLEU for MultiWOZ and BLEU/F1 for WoW) are commonly used in past works and they are easy to implement. I am eager to see these scores after seeing the impressive human evaluation results.

* Knowledge retrieval, as the preceding step of response generation, can have a large impact on the quality of generated responses. However, the paper did not provide any information on the performance (e.g. accuracy/f1 against golden knowledge) of its knowledge source (GPT2-large), which makes it difficult to analyze which module contributes the most to the improvement over baselines.

* An infamous feature of gradient-based decoding is its inefficiency. The paper should list each model's running time/cost at least for inference, especially when gradient-based decoding is used not only for the response generator (BART) but also the knowledge source (GPT2-large).

* The review of related works is incomplete. Gradient-based decoding works (e.g. [1][2][3]) should have been thoroughly discussed since it composes the basic idea of this paper.

[1] Plug and Play Language Models: A Simple Approach to Controlled Text Generation.
[2] Plug-and-Play Conversational Models.
[3] Back to the Future: Unsupervised Backprop-based Decoding for Counterfactual and Abductive Commonsense Reasoning.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
* A simple, intuitive, and effective proposal on injecting knowledge into dialog models without finetuning.

* Extremely good empirical results.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
* Automated evaluation for quality is not presented.

* The performance of the knowledge retrieval module is unknown.

* Efficiency of the model is not presented.

* The literature review is incomplete.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
1. According to the PPLM paper, the input logits to BoW loss should be from the generated text part.
However, in line 234, the authors say {Wz_1...Wz_T} are used as logits for computing BoW CE against knowledge snippet tokens {k1, ..., kT}, which implies the logits have the same length as the knowledge snippet. 
Can the authors clarify what the input to BoW loss is? Is it logits of the generated response (on the decoder side) or logits computed from the encoded knowledge snippet (on the decoder side)?

2. Is the knowledge source GPT2-large finetuned on MultiWOZ or WoW?

3. Is the baseline BART finetuned on WoW?

4. Does baseline BART use the same knowledge source as POKI?
---------------------------------------------------------------------------


Missing References
---------------------------------------------------------------------------
Plug-and-Play Conversational Models. EMNLP Findings 2020.
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 1
     Overall Recommendation - Long Paper: 2.5


============================================================================
                            REVIEWER #2
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
In order to improve the specificity and informativeness of generated responses of dialogue systems, the authors propose a knowledge-injection method and use gradient-based inference to augment generated responses with extracted knowledge from external sources at decoding time. Their method achieves better performance considering both automatic and human evaluation and does not require any additional training for knowledge injection.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
1.The knowledge-injection technique they proposed is adaptable to any dialogue response generation model because it doesnâ€™t require any additional training to leverage external knowledge compared to existing works (training-agnostic). 

2.They provide detailed and comprehensive human evaluation and achieve better performance compared with baselines.

3.The general idea makes sense.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
1.In the parametric knowledge extraction, the prompts are created manually and there are only 9 templates as the prompts. Such usage limits the diversity of knowledge extraction. Itâ€™s better to conduct a statistical analysis to show â€œhow many extracted knowledge comes from the parametric knowledge extraction, and how many knowledge comes from non-parametric methodsâ€ .

2.The proposed method is not novel enough. Both knowledge extraction and gradient-based decoding methods largely depend on existing tools or works.

3.In general, the experiments make sense. However, some parts of the experiments are not so convincing. In the automatic evaluation, this paper only considers â€˜diversityâ€™ and ignores some other important aspects (e.g. fluency by PPL, the matching with ground-truth by BLEU, NIST, Rouge, or Bert-based similarity, the semantic matching with input utterance by Bert-based similarity). The authors do not need to consider all aspects I mentioned above, but only one aspect â€˜diversityâ€™ is not enough.
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 4
     Overall Recommendation - Long Paper: 3


============================================================================
                            REVIEWER #3
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
The paper concerns the augmentation of machine responses in
task-oriented (MultiWOZ) and knowledge-grounded (WOW) dialog models
with extra specific relevant information from snippets obtained from a
pretrained GPT-2 language model fine-tuned with Hearst-pattern-like
templates or "prompts" in a system POKI.  In both cases,
gradient-based decoding is applied using soft constraints to keep the
responses consistent and non-redundant with the dialog history,
distinctively including the initial response of the supervised model, and to
ensure conservation of the retrieved information.  The soft constraints
include the use of entailment and cross entropy loss, and a language
model to ensure fluency.  Evaluation of the ensuing dialogs uses
state-of-the-art dialog models in the task- and knowledge- oriented
domains as baselines, using both automatic measures of n-gram
diversity and entropy of dialogs and human evaluations in terms of
scalar coherence, informativity, etc.  There is also a Bot-play
evaluation of the dialog as a whole, in which a version of the
DialoGPT model of Zhang et al fine-tuned on human-user utterances acts
as a proxy for real users, and human annotators estimate how
successfully the dialog as a whole scores in comparison with the
various baselines, including the gold dialogs, on the "conversational
goal".  It is claimed in the abstract and introduction on the basis of
this measure that POKI augmentation of responses helps to achieve the
conversational goals.  

The automatic measures show that on both dialog-domains, not too
surprisingly, the soft constraints induce dialog responses that have
higher unigram and bigram diversity and higher entropy than the
baseline of simply appending snippets to the initial moves of the
models (KCopy), and over the gold data.   They 
also score better on these measures in comparison to the relevant SoA
models including  various versions of Sun et al 2021 for
MultiWOZ and BART for WOW.  Ablation shows entailment to be less
important than completeness on these measures.

Human judgements of the utterance-level
quality of the dialogs on the various dimensions in comparison to the
same baselines shows startlingly consistent superiority of POKI
augmentation, with kappa scores to indicate confidence.  However, the fact
that gold responses score *less* highly on MultiWOZ than POKI on the
dimensions of coherence, informativity, human-likeness, and
usefulness, as well as on the latter two dimension for WOW, makes one
wonder what these judgements are actually assessing.  As the paper
admits in section 5.1, these dimensions might reflect other properties of the 
utterances than objective conversational success on the those
specified.  Ablation again suggests theat entailment is less important
than completeness.

The Bot-play measure is claimed to give a more global assessment of
the dialog as a whole.  However, this measure is not clearly defined
in section 5. In particular, the role of the DialoGPT model of the
user is as noted unclear, and the "conversational goal" differs across
the two dialog types.  In the case of TOD, the onversational goal is
naturally the achievement of the task, and the gold dialog and POKI
are judged to be similarly effective.  While POKI seems to be somewhat
preferred to other models, kappa scores across the various comparisons
are depressed.  In the case of knowledge-oriented dialog, the
conversational goal is necessarily defined differently, as "sustaining
a longer and engaging dialog."  Of the comparison models, BART scores
as highly as POKI, and gold dialog is again judged to be similarly effective
to POKI.  It isn't clear on the basis of these results that the claim
for response augmentation as of positive help in achieving concrete
conversational goals such as task completion is justified.

More generally, the idea that users will find dialog augmented by
generation from a huge language model more appealing than dialog
narrowly constrained by necessarily limited knowledge embodied in the
training data itself is reasonable, and the specific tactic of
generating from the supervised model response makes sense.  It is less
clear that the augmentation is of any more practical use than the
chat-bots it resembles, or more fundamentally that it can affect the
quality of the information conveyed in the dialog in the way that is
claimed.

Details:

References:  Dinan 2019 a and b are the same
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
See review
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
See review
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 3
     Overall Recommendation - Long Paper: 2


==> files/todos.tex <==
New points to add in emnlp paper (taken from slack):
— add new baselines
— try something more for prompt engineering
— expand the bot-play evaluation with clearer description of conversational goals
— add automatic metrics for generation
— add performance for knowledge retrieval
— perform speed analysis and compare with other models


Knowledge generation / extraction Analysis
- human eval for retrieval
- recall at K, ngram overlap - topic? entity? CIDER, ROUGE
- parametric vs non-parametric contribution
- NLI based metrics if possible, not high priority (MNLI)
- Adding previous conversation as another non-parametric source
- Factually correct, sanity check: parametric vs non-parametric


some rewriting in intro
- why knowledge injection is useful. more references
- rewriting/editing the contributions

a. We identified that knowledge injection is useful in goal-oriented dialog and KG dialog. We show a simple method of knowledge injection at inference. doesn't involve retraining the model (diff from all previous works)
b. automatic and human eval shows that our method is helpful
c. real user study shows that it can actually help people to achieve their goal better

Experiment section can be broken down with research qs
---------------------------------------------------------------------------

reviews

using external knowledge
    - r3: gold is rated as worse
    - emphasize this point more in intro/motivation/experiments

table 3 
    - add win/loss as opposed to win/tie [to address r3 confusion]
    
    
r3 'It is less
clear that the augmentation is of any more practical use than the chat-bots it resembles, or more fundamentally that it can affect the quality of the information conveyed in the dialog in the way that is claimed.'


Write dataset names instead of gold

----------------------------------------------------------------------
Julian's reply:

The first highlighted part seems to basically just be saying "if you're doing better than 'gold', then what does the evaluation criterion really assess?". Or alternately, what does the "gold" really represent if you can do better than it? I think you need to explain here why it makes sense that you're able to do better than gold (e.g. because you're including additional information that's not part of what's used to generate the gold data). Without a deeper explanation I can agree that it's a bit head-scratchy to be able to do better than "gold" for some task -- either it means the evaluation is funny, or that gold is not gold.

For the second point, they seem to just be saying that you can come up with something cool that people will like, but that doesn't really prove that it'll actually help people to achieve some goal more rapidly. I think this is a general criticism with a lot of research where people design a "fancier" model than some alternative. Users will say "yeah this is better!" but you're not actually proving it helped them to *do* anything more accurately or more efficiently.

At least that's my take from a quick read (and not remembering perfectly which parts of the paper it corresponds to). What's your take?

I think the basic idea (regardless of other confusion which you can probably correct) is that they doubt the injected knowledge will really *help* users to do anything. Hard to test that without giving users "real" conversational goals and having them actually engage in conversations (rather than evaluating existing conversations). Otherwise you're arguably just testing whether evaluators think the thing looks cool. That'd be a pretty tough experiment to conduct, and if you're not willing to it may be fair to concede that point, and say instead that your argument is that they're (a) subjectively good, according to users; (b) useful, as argued by results of bot-play experiments (I think?); the latter is maybe less convincing though.

It needn't be more than e.g. low 10s of users.


%%%% H:
% overall. flag any portions not critical. reviewer hat.
% overall structure
% method section. equation.
% intro . more text/references for knowledge injection.
% retrieval study ideas / analysis 
